Two-particle Bose-Einstein correlations in $pp$ collisions at $\mathbf {\sqrt{s} =}$ 0.9 and 7 TeV measured with the ATLAS detector

The paper presents studies of Bose-Einstein Correlations (BEC) for pairs of like-sign charged particles measured in the kinematic range $p_{\rm T}>$ 100 MeV and $|\eta|<$ 2.5 in proton--proton collisions at centre-of-mass energies of 0.9 and 7 TeV with the ATLAS detector at the CERN Large Hadron Collider. The integrated luminosities are approximately 7 $\mu$b$^{-1}$, 190 $\mu$b$^{-1}$ and 12.4 nb$^{-1}$ for 0.9 TeV, 7 TeV minimum-bias and 7 TeV high-multiplicity data samples, respectively. The multiplicity dependence of the BEC parameters characterizing the correlation strength and the correlation source size are investigated for charged-particle multiplicities of up to 240. A saturation effect in the multiplicity dependence of the correlation source size is observed using the high-multiplicity 7 TeV data sample. The dependence of the BEC parameters on the average transverse momentum of the particle pair is also investigated.

==> STDM-2013-01_title.tex <==

 Two-particle Bose--Einstein correlations in $pp$ collisions at $\mathbf {\sqrt{s} =}$  
0.9 and 7 TeV measured with the ATLAS detector



The paper   presents studies of Bose--Einstein Correlations (BEC) for pairs of   
like-sign  charged particles measured in the kinematic  range $p_{\rm T} >$ 100 MeV and $|\eta|<$ 2.5  
in   proton--proton   collisions at centre-of-mass energies of 0.9  and 7 TeV with the 
ATLAS detector at the CERN Large Hadron Collider. 
The integrated luminosities are  approximately 7 $\mu$b$^{-1}$,   190 $\mu$b$^{-1}$  and   12.4 nb$^{-1}$ 
 for   0.9 TeV,  7 TeV minimum-bias  and 7 TeV  high-multiplicity  data samples,   respectively.
The multiplicity dependence of the BEC  parameters characterizing the  correlation strength 
and the correlation source size  are investigated for charged-particle  multiplicities of up to 240. 
A saturation effect in the multiplicity dependence of the correlation source size is observed  using the  high-multiplicity  
7 TeV data sample.  
The dependence of the BEC parameters  on the average transverse momentum of the  particle pair  is  also   investigated.   

